Enhancing LLMs for Identifying and Prioritizing Important Medical Jargons from Electronic Health Record Notes Utilizing Data Augmentation: A Comparative Study

OpenNotes gives patients access to their EHR notes, but dense medical jargon limits comprehension. We evaluate closed-source and open-source LLMs for extracting and prioritizing the jargon terms most relevant to individual patients, using 90 expert-annotated EHR notes. We test combinations of general vs. structured prompts, zero-shot vs. few-shot prompting, fine-tuning, and GPT-4o-based data augmentation, the last paired with a ranking technique to refine training in low-resource settings. To assess the effect of dataset size, we fine-tune on augmented datasets scaled from 10 to 9,995 examples. All settings are evaluated with 10-fold cross-validation, reporting F1 and Mean Reciprocal Rank (MRR) under two string-matching criteria (relaxed matching and Jaccard Index), followed by an error analysis of model outputs. Open-source models performed best when fine-tuned on the gold-standard dataset: under Jaccard-based matching, DeepSeek 8B achieved the top F1 (0.431, SD 0.046) and BioMistral 7B the top MRR (0.577, SD 0.109). Under relaxed matching, however, open-source models did not match closed-source performance even with augmentation or fine-tuning. Few-shot prompting offered no advantage over zero-shot in vanilla models; prompting style substantially affected results; fine-tuning on a small gold-standard set improved performance; and data augmentation matched or exceeded fine-tuning, though its benefit depended heavily on augmented-data quality. These findings show that prompting strategy, fine-tuning, and data augmentation each meaningfully improve LLM performance on patient-centered jargon extraction in low-resource clinical settings.

==> old.tex <==
\pagebreak
\section*{Snippet of Discharge Note}
\begin{figure}[!ht]
    \centering
\begin{tcolorbox}
Name:  \_\_\_                     Unit No:   \_\_\_
 
Admission Date:  \_\_\_              Discharge Date:   \_\_\_
 
Date of Birth:  \_\_\_             Sex:   F
 
Service: MEDICINE
 
Allergies: 
No Known Allergies / Adverse Drug Reactions
 
Attending: \_\_\_
 
Chief Complaint:
Worsening ABD distension and pain 
 
Major Surgical or Invasive Procedure:
Paracentesis
\\
History of Present Illness: \\
\_\_\_ HCV cirrhosis c/b ascites, hiv on ART, h/o IVDU, COPD, 
bioplar, PTSD, presented from OSH ED with worsening abd 
distension over past week.  
Pt reports self-discontinuing lasix and spirnolactone \_\_\_ weeks 
ago, because she feels like "they don't do anything" and that 
she "doesn't want to put more chemicals in her." She does not 
follow Na-restricted diets. In the past week, she notes that she 
has been having worsening abd distension and discomfort. She 
denies \_\_\_ edema, or SOB, or orthopnea. She denies f/c/n/v, d/c,
dysuria. She had food poisoning a week ago from eating stale 
cake (n/v 20 min after food ingestion), which resolved the same 
day. She denies other recent illness or sick contacts. She notes 
that she has been noticing gum bleeding while brushing her teeth 
in recent weeks. she denies easy bruising, melena, BRBPR, 
hemetesis, hemoptysis, or hematuria.  \\
Because of her abd pain, she went to OSH ED and was transferred 
to \_\_\_ for further care. Per ED report, pt has brief period of 
confusion - she did not recall the ultrasound or bloodwork at 
osh. She denies recent drug use or alcohol use. She denies 
feeling confused, but reports that she is forgetful at times.  
In the ED, initial vitals were 98.4 70 106/63 16 97\%RA  
Labs notable for ALT/AST/AP \_\_\_ \_\_\_: \_\_\_, 
Tbili1.6, WBC 5K, platelet 77, INR 1.6  \\
...\\
Discharge Instructions:
Dear Ms. \_\_\_,
It was a pleasure taking care of you! You came to us with 
stomach pain and worsening distension. While you were here we 
did a paracentesis to remove 1.5L of fluid from your belly. We 
also placed you on you 40 mg of Lasix and 50 mg of Aldactone to 
help you urinate the excess fluid still in your belly. As we 
discussed, everyone has a different dose of lasix required to 
make them urinate and it's likely that you weren't taking a high 
enough dose. Please take these medications daily to keep excess 
fluid off and eat a low salt diet. You will follow up with Dr. 
\_\_\_ in liver clinic and from there have your colonoscopy 
and EGD scheduled. Of course, we are always here if you need us. 
We wish you all the best!
Your \_\_\_ Team.  
 
Followup Instructions:
\_\_\_

\end{tcolorbox}
    \caption{MIMIC-IV discharge note}
    \label{mimic_notes}
\end{figure}
